Heavy-Traffic Analysis of Queueing Systems with no Complete Resource Pooling

We study the heavy-traffic limit of the generalized switch operating under MaxWeight, without assuming that the CRP condition is satisfied and allowing for correlated arrivals. The main contribution of this paper is the steady-state mean of linear combinations of queue lengths in heavy traffic. We showcase the generality of our result by presenting various stochastic networks as corollaries, each of which is a contribution by itself. In particular, we study the input-queued switch with correlated arrivals and we show that if the state space collapses to a full-dimensional subspace, the correlation among the arrival processes does not matter in heavy traffic. We exemplify this last case with a parallel-server system, an N-system, and an ad hoc wireless network. While the above results are obtained using the drift method, we additionally present a negative result showing a limitation of the drift method. We show that it is not possible to obtain the individual queue lengths using the drift method with polynomial test functions. We do this by presenting an alternate view of the drift method in terms of a system of linear equations, and we use this system of equations to obtain bounds on arbitrary linear combinations of the queue lengths.

==> 1app-details-syst-eqns-proof.tex <==
In this section we prove the claims we made in the proof of Theorem \ref{s.theorem:2switch}.

%\begin{claim*}
%	Consider the queueing system described in Theorem \ref{s.theorem:2switch}. Then,
%	\begin{align*}
%	\E{\qbar_{\perp 1,1}^+\ubarparij{1,1}}\text{ is }O(\sqrt{\epsilon})
%	\end{align*}
%\end{claim*}
\begin{proof}(of Claim \ref{switch.claim.qperp.upar})
	Observe
	\begin{align*}
		\E{\qbar_{\perp 1,1}^+\ubarparij{1,1}}\leq&  \E{\left|\qbar_{\perp 1,1}^+\right| \left|\ubarparij{1,1}\right|} \\
		\leq& \E{\sum_{i=1}^2 \sum_{j=1}^2 \left|\qbar_{\perp i,j}^+\right|\left|\ubarparij{i,j}\right|} \\
		\stackrel{(a)}{\leq}& \sqrt{\E{\left\|\vqbarperp \right\|^2} \E{\left\|\vubar_{\parallel} \right\|^2}} \\
		\stackrel{(b)}{\leq}& \sqrt{T_2}\sqrt{\E{\left\|\vubar_{\parallel} \right\|^2}},
	\end{align*}
	where $(a)$ holds by Cauchy-Schwarz inequality; and $(b)$ holds by Proposition \ref{s.prop:ssc}. Similarly,
	\begin{align*}
	\E{\qbar_{\perp 1,1}^+\ubarparij{1,1}}\geq& - \E{\left|\qbar_{\perp 1,1}^+\right| \left|\ubarparij{1,1}\right|}
	\geq -\sqrt{T_2}\sqrt{\E{\left\|\vubar_{\parallel} \right\|^2}}.
	\end{align*}
	Then,
	\begin{align*}
		\left|\E{\qbar_{\perp 1,1}^+\ubarparij{1,1}}\leq \right|\leq \sqrt{T_2}\sqrt{\E{\left\|\vubar_{\parallel} \right\|^2}} 
	\end{align*}
	and $\E{\left\|\vubar_{\parallel} \right\|^2}$ is $O(\epsilon)$. This proves the claim.
\end{proof}

Now we prove Claim \ref{switch.claim.q11u22}

%\begin{claim}
%	Consider the queueing system described in Theorem \ref{s.theorem:2switch}. Then,
%	\begin{align*}
%	\E{\qbar_{1,1}^+\ubar_{2,2}}= \E{\qbar_{1,2}^+\ubar_{2,2}}+\E{\qbar_{2,1}^+\ubar_{2,2}} + O(\sqrt{\epsilon}).
%	\end{align*}
%\end{claim}

\begin{proof}(of Claim \ref{switch.claim.q11u22})
	We use Claim \ref{switch.claim.qperp.upar}. We obtain
	\begin{align*}
		\E{\qbar_{1,1}^+\ubar_{2,2}}=& \E{\qbarparij{1,1}^+\ubar_{2,2}} + O(\sqrt{\epsilon}) \\
		\stackrel{(a)}{=}& \E{\left(\qbarparij{1,2}^+ +\qbarparij{2,1}^+ - \qbarparij{2,2}^+\right)\ubar_{2,2}} + O(\sqrt{\epsilon}) \\
		\stackrel{(b)}{=}& \E{\left(\qbar_{1,2}^+ +\qbar_{2,1}^+ - \qbar_{2,2}^+\right)\ubar_{2,2}} + O(\sqrt{\epsilon}) \\
		\stackrel{(c)}{=}& \E{\left(\qbar_{1,2}^+ +\qbar_{2,1}^+  \right)\ubar_{2,2}} + O(\sqrt{\epsilon})
	\end{align*}
	where $(a)$ holds by Equation \eqref{s.2.eq.ssc2}; $(b)$ holds by the previous claim; and $(c)$ holds by Equation \eqref{s.eq.qu}.
\end{proof}

==> 1app-gs-lemma-bound.tex <==
\begin{proof}[of Lemma \ref{gs.lemma:bound}]
For each $m\in\cM$, let $\thetam\in\left(0,\tfrac{\pi}{2} \right]$ be such that 
\begin{align*}
	\langle\vcl,\vsbar\rangle=\bml\quad\text{if and only if}\quad\dfrac{\left\|\vqbarparh \right\|}{\left\|\vqbar \right\|}\geq \cos\left(\thetam\right). 
\end{align*}
Let $\ds\thetamin=\min_{m\in \cM}\{\thetam\}$ and $\thetaq$ be the angle between $\vqbar$ and $\vqbarparh$. Then,
\begin{align*}
	\cos(\thetaq)=\dfrac{\left\|\vqbarparh \right\|}{\left\|\vqbar \right\|}
\end{align*}
and
\begin{align*}
	\langle \vcl,\vsbar\rangle \neq \bml\quad\text{if and only if}\quad \thetam<\thetaq
\end{align*}

By definition of $\bml$ we have
\begin{align*}
	0\geq& \sum_{\ell\in P}\sum_{m\in\cM}\psi_m\Em{
		\left. \xi_\ell \left(\langle\vcl,\vsbar\rangle-\bml \right) \right|\langle\vcl,\vsbar\rangle\neq\bml } \left(1-\piml\right) \\
	\stackrel{(a)}{\geq}& \E{\left\|\vqbarparh \right\|\sum_{\ell\in P}\sum_{m\in\cM} \psi_m \Em{\left. \langle\vcl,\vsbar\rangle-\bml  \right|\langle\vcl,\vsbar\rangle\neq\bml}} \left(1-\piml\right)  \\
	=& \E{\left\|\vqbar \right\|\cos(\thetaq) \sum_{\ell\in P}\sum_{m\in \cM}\psi_m \Em{\left.\langle\vcl,\vsbar\rangle-\bml \right| \langle\vcl,\vsbar\rangle\neq\bml}} \left(1-\piml\right) \\
	\stackrel{(b)}{=}& \E{\left\|\vqbarperph \right\|\cot(\thetaq) \sum_{\ell\in P} \sum_{m\in \cM}\psi_m \Em{\langle\vcl,\vsbar\rangle-\bml \ind{\langle\vcl,\vsbar\rangle\neq\bml}} } \\
	\stackrel{(c)}{\geq}& \cot\left(\thetamin\right)\E{\left\|\vqbarperph \right\| \sum_{\ell\in P} \sum_{m\in \cM}\psi_m \Em{\langle\vcl,\vsbar\rangle-\bml} } \\
	\stackrel{(d)}{=}& \cot\left(\thetamin\right)\E{\left\|\vqbarperph \right\|\sum_{\ell\in P} \left(\langle \vcl,\vs\rangle-\bl\right)} \\
	\stackrel{(e)}{\geq}& -\cot\left(\thetamin\right)\sqrt{\E{\left\|\vqbarperph \right\|^2}\E{\left(\sum_{\ell\in P}\langle\vcl,\vsbar\rangle-\bl \right)^2} } \\
	\stackrel{(f)}{\geq}& -\widetilde{\zeta}\sqrt{\epsilon}
\end{align*}
where $\widetilde{\zeta}$ is a nonnegative finite constant and  $(a)$ holds because $\xi_\ell$ is the norm of the projection of $\vqbar$ on $\vcl$, so $\xi_\ell\leq \left\|\vqbarparh \right\|$; $(b)$ holds because $\vqbar$, $\vqbarparh$ and $\vqbarperph$ form a right triangle, and by definition of conditional expectation; $(c)$ holds because $f(x)=\cot(x)$ is nondecreasing for $x\in\left(0,\tfrac{\pi}{2} \right]$, $\ind{\langle\vcl,\vsbar\rangle\neq \bml}\leq 1$ with probability 1 and $\bml-\langle\vcl,\vsbar\rangle\leq 0$ with probability 1; $(d)$ holds because $\E{\bml}=\bl$; $(e)$ holds by Cauchy-Schwarz inequality; and $(f)$ holds because by SSC in Proposition \ref{gs.prop:gen.switch.SSC} we have $\E{\left\|\vqbarperph\right\|^2}\leq T_2$ where $T_2$ is a finite constant, and because
\begin{align*}
	0\leq& \E{\left(\sum_{\ell\in P}\langle\vcl,\vsbar\rangle-\bl \right)^2} \\
	\stackrel{(*)}{\leq} & \sum_{m\in\cM}\psi_m \Em{\left. \sum_{\ell\in P}\left(\langle\vcl,\vsbar\rangle-\bml \right)^2 \right|\langle\vcl,\vsbar\rangle\neq \bml} \left(1-\piml\right) \\
	\leq& \sum_{m\in \cM}\psi_m\sum_{\ell\in P} \left(\vcl,\vone \smax\rangle + \bml \right)^2 \dfrac{\bml}{\gammam}\epsilon
\end{align*}
where $(*)$ holds because given $\Mbar=m$, $\langle\vcl,\vsbar\rangle-\bml\leq 0$ with probability 1. 

This proves the lemma.
\end{proof}

==> 1app-gs-sv-Oe.tex <==
\proof{Proof of Equation \eqref{gs.eq.s-v.Oe}.}
We need to prove that
\begin{align*}
	\E{\left\|\vsbar-\vnu \right\|^2\ind{\vsbar\notin \cap_{\ell\in P}\cF^\pl}}\text{ is $O(\epsilon)$}.
\end{align*}

First observe that if $\theta^\pl \in\left[0, \frac{\pi}{2} \right]$ is the angle between $\vsbar-\vnu$ and $\vcl$, then 
\begin{align*}
	\left\|\vsbar-\vnu \right\|= \dfrac{|\langle\vcl,\vsbar-\vnu\rangle|}{\cos\left(\theta^\pl \right)}.
\end{align*}

Observe that for any $\ell\in P$ we have
\begin{align}
	& \E{\dfrac{\left| \langle \vcl,\vsbar-\vnu\rangle\right|}{\cos\left(\theta^\pl \right)}\ind{\vsbar\notin \cF^\pl}} \nonumber \\
	\stackrel{(a)}{=}& \E{\dfrac{\left|\langle\vcl,\vsbar\rangle - \bl\right|}{\cos\left(\theta^\pl \right)}\ind{\vsbar\notin \cF^\pl}} \nonumber \\
	\stackrel{(b)}{=}& \sum_{m\in\cM}\psi_m \Em{\left. \dfrac{\left|\langle\vcl,\vsbar\rangle-\bml\right|}{\cos\left(\theta^\pl \right)}\ind{\vsbar\notin \cF^\pl} \right| \langle\vcl,\vsbar\rangle\neq \bml} \left(1-\piml\right) \nonumber \\
	\stackrel{(c)}{=}& O(\epsilon), \label{gs.eq.theta.epsilon}
\end{align}
where $(a)$ holds because $\vnu\in \cF^\pl$ for all $\ell\in P$; $(b)$ holds by conditioning on the channel state and by definition of $\piml$ in Lemma \ref{gs.lemma:cl.s.bl}; and $(c)$ holds by Lemma \ref{gs.lemma:cl.s.bl} and because $\vsbar$, $\vcl$ and $\vnu$ are bounded vectors, and $\cos\left(\theta^\pl\right)\neq 0$ under the condition $\vsbar\notin \cF^\pl$.

Therefore, we obtain
\begin{align*}
	0\leq& \E{\left\|\vsbar-\vnu \right\|^2 \ind{\vsbar\notin \cap_{\ell\in P}\cF^\pl} } \\
	\stackrel{(a)}{\leq}& \left(n\smax+\sum_{i=1}^n \nu_i \right)\E{\left\|\vsbar-\vnu \right\| \ind{\vsbar\notin\cap_{\ell\in P}\cF^\pl}} \\
	\stackrel{(b)}{=}& \left(n\smax+\sum_{i=1}^n \nu_i \right)\E{\dfrac{\left|\langle\vc^{(\tilde{\ell})},\vsbar-\vnu\rangle\right|}{\cos(\theta^{(\tilde{\ell})})} \ind{\vsbar\notin\cap_{\ell\in P}\cF^\pl}} \\
	\stackrel{(c)}{=}& O(\epsilon)
\end{align*}
where $\tilde{\ell}\in P$ is such that $\vsbar\notin \cF^\pl$ conditioned on $\vsbar\notin \cap_{\ell\in P}\cF^\pl$. Here, $(a)$ holds because $\sbar_i\leq \smax$ with probability 1 and because $\sbar_i-\nu_i\leq \sbar_i+\nu_i$ for all $i\in[n]$ because both vectors have nonnegative elements; and $(c)$ holds by Equation \eqref{gs.eq.theta.epsilon}. 

This completes the proof.
\Halmos
\endproof

==> 1app-hajek-lemma.tex <==
We state a Lemma that was first proved in \cite{hajek_drift} in a more general setting, and that is useful to prove SSC.

\begin{lemma}\label{lemma:hajek}
	For an irreducible and aperiodic Markov Chain \newline $\left\{X(k):k\geq 1\right\}$ over a countable state space $\cX$, suppose $Z:\cX\to \bR_+$ is a nonnegative valued Lyapunov function. Define the drift of $Z$ at $x$ as
	\begin{align}\label{gs.eq.def.drift}
		\Delta Z(x)\defn \big[Z\left(X(k+1)\right)-Z\left(X(k)\right) \big]\ind{X(k)=x}.
	\end{align}
	Thus, $\Delta Z(x)$ is a random variable that measures the amount of change in the value of $Z$ in one time slot, starting from state $x$. If the following conditions are satisfied
	\begin{itemize}
		\item[(C1)] There exists $\eta>0$ and $\tau<\infty$ such that
		\begin{align*}
			\E{\Delta Z(x)\,|\, X(k)=x}\leq -\eta\qquad\text{for all $x\in \cX$ with $Z(x)\geq \tau$}
		\end{align*}
		
		\item[(C2)] There exists $D<\infty$ such that
		\begin{align*}
			\Prob{|\Delta Z(x)|\leq D}=1\qquad\text{for all $x\in \cX$}
		\end{align*}
	\end{itemize}
	
	Then, there exist $\theta^\star>0$ and $C^\star<\infty$ such that
	\begin{align*}
		\limsup_{k\to\infty}\E{e^{\theta^* Z(X(k))}}\leq C^*
	\end{align*}
	
	Further, if the Markov chain $\{X(k): k\geq 1\}$ is positive recurrent, then $Z(X(k))$ converges in distribution to a random variable $\overline{Z}$ for which
	\begin{align*}
		\E{e^{\theta^* \overline{Z}}}\leq C^*,
	\end{align*}
	which directly implies that the moments of $\overline{Z}$ exist and are finite.
\end{lemma}


==> 1app-proj-K.tex <==
By definition of the cone $\cK$ in \eqref{s.eq.cone}, for any $\vy\in\bR^{2^2}$ we have
	\begin{align}
		& \begin{aligned}\label{s.2.eq.par11} 
			y_{\parallel 1,1}=& \dfrac{y_{1,1}+y_{1,2}}{2}+ \dfrac{y_{1,1}+y_{2,1}}{2}-\dfrac{y_{1,1}+y_{1,2}+y_{2,1}+y_{2,2}}{4} \\
			=& \dfrac{3y_{1,1}+y_{1,2}+y_{2,1}-y_{2,2}}{4}
		\end{aligned} \\
		& \begin{aligned}\label{s.2.eq.par12}
			y_{\parallel 1,2}=& \dfrac{y_{1,1}+y_{1,2}}{2}+ \dfrac{y_{1,2}+y_{2,2}}{2}-\dfrac{y_{1,1}+y_{1,2}+y_{2,1}+y_{2,2}}{4} \\
			=& \dfrac{y_{1,1}+3y_{1,2}-y_{2,1}+y_{2,2}}{4}
		\end{aligned}  \\
		& \begin{aligned}\label{s.2.eq.par21}
			y_{\parallel 2,1}=& \dfrac{y_{2,1}+y_{2,2}}{2}+ \dfrac{y_{2,1}+y_{1,1}}{2}-\dfrac{y_{1,1}+y_{1,2}+y_{2,1}+y_{2,2}}{4} \\
			=& \dfrac{y_{1,1}-y_{1,2}+3y_{2,1}+y_{2,2}}{4} .
		\end{aligned}
	\end{align}
	Then, since the switch is completely saturated we have
	\begin{align}\label{s.2.eq.Ea}
		\E{\abarparij{i,j}}=& \dfrac{1-\epsilon}{2}+\dfrac{1-\epsilon}{2}-\dfrac{2(1-\epsilon)}{4}=\dfrac{1-\epsilon}{2} \qquad\forall i,j\in[2]
	\end{align}
	and since $\vsbar$ is a maximal schedule we have
	\begin{align}\label{s.2.eq.spar}
		\sbarparij{i,j}=& \dfrac{1}{2}+\dfrac{1}{2}-\dfrac{2}{4}=\dfrac{1}{2}\qquad\forall i,j\in[2].
	\end{align}
